FairRAG: Fair Human Generation via Fair Retrieval Augmentation

Existing text-to-image generative models reflect or even amplify societal biases ingrained in their training data. This is especially concerning for human image generation where models are biased against certain demographic groups. Existing attempts to rectify this issue are hindered by the inherent limitations of the pre-trained models and fail to substantially improve demographic diversity. In this work, we introduce Fair Retrieval Augmented Generation (FairRAG), a novel framework that conditions pre-trained generative models on reference images retrieved from an external image database to improve fairness in human generation. FairRAG enables conditioning through a lightweight linear module that projects reference images into the textual space. To enhance fairness, FairRAG applies simple-yet-effective debiasing strategies, providing images from diverse demographic groups during the generative process. Extensive experiments demonstrate that FairRAG outperforms existing methods in terms of demographic diversity, image-text alignment, and image fidelity while incurring minimal computational overhead during inference.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/old5_results.tex <==
\section{Results}

\subsection{Overall Results}
\begin{figure*}[]
\footnotesize
 \centering
    \includegraphics[width=0.9\textwidth]{images/comparison_programmer.pdf}
  \caption{Example outputs from each comparison method for the text prompt \textit{Photo of a computer programmer}. Baseline methods, barring Text Augmentation, fail to produce images with high demographic diversity. \gls{FRAG} improves demographic diversity with the help of external visual references. Apart from that, it also improves alignment and fidelity.}
\label{fig:qual_comp}
\end{figure*}
\label{sec:results_overall}
\input{tables/main_results}
In this section, we discuss the overall qualitative and quantitative results. Fig.~\ref{fig:qual_comp} shows example outputs from different methods. Table~\ref{tab:overall_results} summarizes the diversity, alignment and fidelity metrics alongside the absolute improvements over \gls{SD}. \gls{FRAG} outperforms all other methods across all of the quantitative metrics, showing the benefits of the proposed setup for human generation. We observe that \gls{FRAG} effectively leverages human-specific attributes from the reference images to condition the generated images, resulting in enhanced demographic diversity. As presented in Table~\ref{tab:diversity}, it is able to improve diversity metrics for all three: age, gender and skin tone attributes. 

In terms of the baselines, we find that \gls{BaseRAG} is also able to improve diversity, alignment and fidelity scores, however, the additional fairness interventions used in \gls{FRAG}, \ie, \textit{fair re-ranking} and the \textit{transfer instruction} help boost the diversity scores further. In terms of non-RAG baselines, we find \gls{TextAug} to be the most effective, obtaining improvements in diversity, image-text alignment and fidelity metrics. However, qualitatively, it produces synthetic, unrealistic contexts as shown in Fig.~\ref{fig:qual_comp}. \gls{FRAG} on the other hand generates more realistic images due to the conditioning from real images. Next, \gls{Interven} and \gls{FairDiff} also improve the diversity scores to some extent, but are well below \gls{FRAG}. As shown in Fig.~\ref{fig:qual_comp}, \gls{Interven}'s extra textual intervention results in grids of smaller sub-images, which is an undesired side-effect. \gls{FRAG} also uses extra textual instruction, but this does not lead to such inadvertent consequences. Therefore compared to the baseline methods, \gls{FRAG} stands out as more effective.



\paragraph{Diversity for different prompt categories.} We present example outputs for different categories in Fig.~\ref{fig:qual_FRAG} and present the diversity metrics in Table~\ref{tab:by_concept_type}. \gls{FRAG} obtains the highest diversity score in each category, showcasing generalization across different professions.

% \subsection{Breakdown of Demographic Diversity}
\input{tables/demographic_diversity}
% The primary focus of \gls{FRAG} is to improve demographic diversity. As such, we present the improvements in age, gender and race diversity values for all of the comparison methods in Table~\ref{tab:diversity}. \gls{FRAG} outperforms rest of the comparison methods on each of those attributes, showing the efficacy of the proposed setup.


\input{tables/by_concept_type}


\begin{figure*}
\footnotesize
 \centering
    \includegraphics[width=0.85\textwidth]{images/different_concept_types.pdf}
  \caption{FRAG improves demographic diversity for different categories of professions.}
\label{fig:qual_FRAG}
\end{figure*}


\subsection{Minimal Increase in Latency}
\gls{FRAG} involves: a) text-to-image retrieval, b) fair re-ranking, c) visual reference projection to obtain the bimodal prompt, and d) conditional image generation. The first three steps are specific to \gls{FRAG}, but add minimal computational overhead. On a single NVIDIA A10G Tensor Core GPU, \gls{SD} and \gls{FRAG} require 2.8 secs and 3 secs respectively, to generate a single image with 20 denoising steps.

\subsection{Face and Body Size}
Most past studies on fairness in generation, focus on close-up views of faces without analyzing half and full body results. Here, we use three different prompt prefixes to control the face and body size: \textit{Headshot of}, \textit{Half body of} and \textit{Full body of}. As shown in Fig.~\ref{fig:face_size}, we find that for half and full body images, \gls{FRAG} tends to generate more realistic contexts than the SDv2.1 baseline. This shows the efficacy of \gls{FRAG} in generating different sizes of humans. However, both the methods also tend to generate disfigurements, \eg, in small faces, fingers and limbs. \gls{FRAG} does not fix this through conditioning and we hypothesize this issue requires other mechanisms for introducing human anatomy prior which may require re-training or tuning the model too, so we leave this to future work.
\begin{figure}[]
\footnotesize
 \centering
    \includegraphics[width=0.48\textwidth]{images/face_size.pdf}
  \caption{While most past works focus on close-up views of faces, we find FRAG performs well on half and full body generation too. (\textcolor{red}{TODO: yet to add the final images})}
\label{fig:face_size}
\end{figure}



\input{tables/ablations}
\subsection{Ablation Studies}
In Table~\ref{tab:ablations}, we present multiple variants of \gls{FRAG} to analyze the effects of fair re-ranking and text instruction. Even in their absence, the framework exhibits enhancements over the \gls{SD} baseline in terms of all the metrics. We observe that text instruction hurts FID score slightly, nevertheless, both text instruction and fair re-ranking contribute positively to the diversity and alignment metrics, thus validating our decisions to incorporate those mechanisms.

\subsection{Number of Retrievals (Top-$N$)}
\label{sec:topN}
\begin{figure}
 \centering
        \includegraphics[width=0.98\linewidth]{images/diversity_vs_clip_topN.pdf}
        \caption{The chart shows the effects of the number of initial retrievals ($N$) on the diversity and alignment scores. We observe a trade-off as the number of candidate $N$ increases, with the diversity score continuing to increase, while CLIP score decreasing after $N=2000$. We thus use $N$ = $2000$ for all of our experiments.}
    \label{fig:topN}
\end{figure}
We assess the impact of the initial retrieval count, $N$ on the diversity and alignment metrics in Fig.~\ref{fig:topN}. Both diversity and CLIP scores increase up to a certain point, here, $N = 2000$. Beyond that, CLIP score declines while the diversity score continues to rise. This trade-off indicates that with increase in retrievals, the representation of demographic groups also increases, but the images selected may lack relevance to the textual prompt, thereby hurting the alignment score. Consequently, we use $N = 2000$ throughout our experiments.



==> tables/ablations_3metrics.tex <==
\begin{table}[]
\centering
\caption{Ablation studies showing how debiased query, balanced sampling and text instruction help boost the diversity score. Also, presenting the metrics for real distribution, showcasing room for improvement.}
\label{tab:ablations_3metrics}
\setlength\tabcolsep{3 pt}
\begin{tabular}{lccc} \hline
\textbf{Method}    & \textbf{Diversity} ($\uparrow$)   & \textbf{CLIP} ($\uparrow$)        & \textbf{FID} ($\downarrow$)         \\ \hline
\gls{SD} & 0.188 & 0.142 & 85.3 \\
\gls{TextAug} & 0.341 & 0.144 & 74.1 \\ \hline
\multicolumn{4}{c}{\textit{Ablated variants of \gls{FRAG}}} \\
\gls{BaseRAG} & 0.374 & 0.146 & 49.4  \\
No Debiased Query & 0.414 & \underline{0.150} & 50.5 \\
No Balanced Sampling & 0.420 & 0.146 & 53.0 \\
No Text Instruction & 0.407 & 0.145 & \underline{48.9} \\
\gls{FRAG} & \underline{0.438} & 0.146 & 51.8 \\ \hline
Retrievals (Real Distr.) & \textbf{0.478} & \textbf{0.158} & \textbf{26.5} \\
\hline
\end{tabular}
\end{table}

==> tables/ablations_for_slides_real.tex <==
\begin{table}[t]
\centering
\caption{Ablation studies showing how debiased query (debiased q), balanced sampling (bal. sampl.) and text instruction (text instr.) help boost the diversity scores. We also present the metrics for retrieved images, \ie, the real distribution, showcasing room for further improvement.}
\label{tab:ablations}
\begin{tabular}{lcccc} \hline
\textbf{Method}      & \textbf{\begin{tabular}[c]{@{}c@{}}Age \end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Gender\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Skin\\ Tone\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Intersec.\end{tabular}} \\ \hline
\gls{SD} & 0.220 & 0.273 & 0.224 & 0.188 \\ 
\gls{FRAG} & \textbf{0.559} & \underline{0.800} & \underline{0.416} & \underline{0.438} \\ 
Retrievals (Real Distribution) & \underline{0.546} & \textbf{0.902} & \textbf{0.526} & \textbf{0.478} \\
\hline
\multicolumn{5}{c}{\textit{Without retrieval-time fairness interventions}} \\
No Debiased Query & 0.525 & 0.764 & 0.411 & 0.414 \\
No Balanced Sampling & \textit{0.538} & 0.734 & 0.392 & 0.420 \\
\multicolumn{5}{c}{\textit{Without generation-time fairness intervention}} \\
No Text Instruction & 0.481 & 0.771 & \underline{0.416} & 0.407 \\ \hline
\end{tabular}
\end{table}

==> tables/ablations_for_slides_wo_real.tex <==

\begin{table}[t]
\centering

\caption{Ablation studies showing how debiased query (debiased q), balanced sampling (bal. sampl.) and text instruction (text instr.) help boost the diversity scores. We also present the metrics for retrieved images, \ie, the real distribution, showcasing room for further improvement.}
\label{tab:ablations}
\begin{tabular}{lcccc} \hline
\textbf{Method}      & \textbf{\begin{tabular}[c]{@{}c@{}}Age \end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Gender\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Skin\\ Tone\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Intersec.\end{tabular}} \\ \hline
\gls{SD} & 0.220 & 0.273 & 0.224 & 0.188 \\ 
\gls{FRAG} & \textbf{0.559} & \textbf{0.800} & \textbf{0.416} & \textbf{0.438} \\ 
\hline
\multicolumn{5}{c}{\textit{Without retrieval-time fairness interventions}} \\
No Debiased Query & 0.525 & 0.764 & \underline{0.411} & 0.414 \\
No Balanced Sampling & \underline{0.538} & 0.734 & 0.392 & \underline{0.420} \\
\multicolumn{5}{c}{\textit{Without generation-time fairness intervention}} \\
No Text Instruction & 0.481 & \underline{0.771} & \textbf{0.416} & 0.407 \\ \hline
\end{tabular}
\end{table}

==> tables/ablations_main_metrics_full_width.tex <==
\begin{table}[]
\centering
\caption{}
\label{tab:ablations}
\begin{tabular}{lcccc} \hline
\textbf{Method}      & \textbf{\begin{tabular}[c]{@{}c@{}}Age \end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Gender\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Skin\\ Tone\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Intersec.\end{tabular}} \\ \hline
\gls{SD} & 0.220 & 0.273 & 0.224 & 0.188 \\
\gls{TextAug} & 0.426 & 0.766 & 0.334 & 0.341 \\ 
\gls{BaseRAG} & 0.440 & 0.562 & \underline{0.437} & 0.386 \\
\hline
\multicolumn{5}{c}{\textit{Ablated variants of \gls{FRAG}}} \\
No Debiased Query for Retrieval & 0.525 & 0.764 & 0.411 & 0.414 \\
No Balanced Sampling for Retrieval & 0.538 & 0.734 & 0.392 & 0.420 \\
No Text Instruction for Generation & 0.481 & 0.771 & 0.416 & 0.407 \\
\gls{FRAG} & \textbf{0.559} & \underline{0.800} & 0.416 & \underline{0.438} \\ \hline
Retrievals & \underline{0.546} & \textbf{0.902} & \textbf{0.526} & \textbf{0.478} \\ \hline
\end{tabular}
\end{table}

==> tables/by_concept_type.tex <==
\begin{table*}[]
\centering
\caption{Overall diversity metrics on the eight concept types used in our evaluation set. \gls{FRAG} shows improvements in each concept type, showcasing the generality of the approach.}
\label{tab:by_concept_type}
\begin{tabular}{lcccccccc} \hline
& \textbf{\begin{tabular}[c]{@{}c@{}}Artists\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}F\&B \\ Workers\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Musicians\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Security \\ Personnel\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Sports \\ Players \end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}STEM \\ Profes.\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}} Workers\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Others\end{tabular}} \\ \hline
\gls{SD} & 0.261 & 0.237 & 0.168 & 0.137 & 0.175 & 0.199 & 0.197 & 0.175 \\
\gls{TextAug} & \underline{0.391} & 0.269 & 0.322 & 0.348 & 0.314 & 0.342 & 0.349 & 0.357 \\
\gls{BaseRAG} & 0.351 & \underline{0.387} & \underline{0.375} & \underline{0.391} & \underline{0.369} & \underline{0.348} & \underline{0.361} & \underline{0.389} \\
\gls{FRAG} & \textbf{0.436} & \textbf{0.413} & \textbf{0.440} & \textbf{0.458} & \textbf{0.416} & \textbf{0.432} & \textbf{0.419} & \textbf{0.454} \\
\hline                      \end{tabular}
\end{table*}

==> tables/main_results_bkp.tex <==
\begin{table*}[]
\centering
\caption{Quantitative results from all the comparison methods, highlighting the methods obtaining the \textbf{best} and the \underline{second-best} scores. Values within the parentheses show the \textcolor{green}{improvement} and \textcolor{red}{deterioration} in terms of absolute difference from the \gls{SD} baseline. Compared to other baselines, FRAG shows improvements in demographic diversity, image-text alignment and image fidelity.}
\label{tab:overall_results}
\begin{tabular}{llll} \hline
\textbf{Methods}      &
\textbf{ Diversity ($\uparrow$)} &
\textbf{CLIP ($\uparrow$)} & \textbf{FID ($\downarrow$)} \\ \hline
\gls{SD} & 0.145 & 0.115 & 84.1 \\
\gls{Interven} & 0.323 (\textcolor{green} {+0.178}) & 0.105 (\textcolor{red} {-0.010}) & 89.8 (\textcolor{red} {+05.7}) \\
\gls{FairDiff} & 0.166 (\textcolor{green} {+0.021}) & 0.116 (\textcolor{green} {+0.001}) & 84.4 (\textcolor{red} {+00.3}) \\
\gls{TextAug} & 0.342 (\textcolor{green} {+0.197}) & 0.124 (\textcolor{green} {+0.009}) & \underline{69.8} (\textcolor{green} {-14.3}) \\
\gls{BaseRAG} & \underline{0.369} (\textcolor{green} {+0.224}) & \underline{0.125} (\textcolor{green} {+0.010}) & \textbf{60.6} (\textcolor{green} {-23.5}) \\
\gls{FRAG} & \textbf{0.427} (\textcolor{green} {+0.282}) & \textbf{0.130} (\textcolor{green} {+0.015}) & \textbf{60.6} (\textcolor{green} {-23.5}) \\
\hline                      \end{tabular}
\end{table*}
